Longest Common Subsequence with Gap Constraints

We consider the longest common subsequence problem in the context of subsequences with gap constraints. In particular, following Day et al. 2022, we consider the setting when the distance (i. e., the gap) between two consecutive symbols of the subsequence has to be between a lower and an upper bound (which may depend on the position of those symbols in the subsequence or on the symbols bordering the gap) as well as the case where the entire subsequence is found in a bounded range (defined by a single upper bound), considered by Kosche et al. 2022. In all these cases, we present effcient algorithms for determining the length of the longest common constrained subsequence between two given strings.

==> alphc.tex.old.tex <==
\paragraph{Solutions for \Problem{LCS-$\Sigma$R}, \Problem{LCS-$\Sigma$L}, and \Problem{LCS-$\Sigma$}.}
\label{sec:alphc}

In general, the solutions to all these problems are based on a dynamic programming approach. We compute an $m \times n$ matrix $M$ such that $M[i,j]=p$ if and only if $p$ is the largest number for which there exists a $(right)$-subsequence (respectively, $(left)$- or $(left,right)$-subsequence) $s_p$ of $v[1:i]$ and $w[1:j]$ such that there are two matching embeddings $e_v$ and $e_w$ of $s_p$ into $v[1:i]$ and $w[1:j]$, respectively, both fulfilling the constraints. The elements of  $M$ can be computed in two ways. On the one hand, we can use Lemma \ref{lem:maxdeq} and get a time complexity of $O(N\sigma)$ (or $O(N\sigma^2)$ for \Problem{LCS-$\Sigma$}). On the other hand, we can use a dynamic version of 2D Range Maximum Queries structures, extending the Sparse Tables from~\cite{BenderF00}, and obtain a time complexity of $O(N\log N)$ (or $O(N\sigma\log N)$ for \Problem{LCS-$\Sigma$}). In all cases, the answer to the considered problems is the maximum element of $M$. For space reasons, our results are described in detail in the full version \cite{AKKMS23}.


==> smallbwin.tex <==
\section{LCS with Global Constraints}
\label{sec:smallbwin}
\vspace*{-0.1cm}


\subsubsection{\Problem{LCS-BR} with small windows.}

In this section, we provide a tool for solving \Problem{LCS-BR} in $O(B 2^B (n + m))$ time.
We note that, while this approach is inefficient for large bounded windows, if there exists some constant $0 < c < 1$ such that, for $B = c \log (n+m)$, this approach provides a subquadratic solution for \Problem{LCS-BR}, running in $O((n+m)^{1+c} \log (n+m))$

This algorithm is split in to two phases.
First, we create two lists, $S_v$ and $S_w$, where $S_v$ (respectively, $S_w$) contains every $B$-subsequence of $v$ (respectively, $w$); a $B$-subsequence may occur multiple times in $S_v$ (or $S_w$), once for each of its embeddings. These two lists are combined to form the list $S$, with each subsequence labelled by the word it originated from.
The list $S$ is then sorted first by length of subsequences (decreasingly, from longest to shortest) then by their lexicographic value, via a radix sort (in $B+1$ passes of the algorithm, one for the length and the rest for each position of the subsequences). Now, the longest common $B$-subsequence of $v$ and $w$ is found by iterating through the sorted $S$ and finding the first pair of consecutive $B$-subsequences $s_1$ and $s_2$ such that $s_1 = s_2$ and $s_1$ and $s_2$ originate from different words.


\begin{lemma}
	\label{lem:Small_B_computation}
	$\Problem{LRC-BR}$ can be solved in $O(B 2^B (n + m))$.
\end{lemma}

\begin{proof}
	Note that there are at most $2^B$ subsequences occurring in the factor $v[i:i+B-1]$, for all $i\in [1, n- B + 1]$. Therefore, it is not hard to see that the list $S_v$, of all $B$-subsequences of $v$, can be constructed in $O(2^B B n)$ time by simply appending to $S_v$, one by one, each subsequence which occurs within the bounded factor $v[i:i+B-1]$, for $i \in [1, n- B + 1]$. We can construct the list $S_w$ in the same way in $O(2^B B m)$ time.

We define the list $S$ as the concatenation of the lists $S_w$ and $S_v$. Clearly, $S$ contains $2^{B}(n + m)$ strings (each of length at most $B$), and can be sorted in $O(2^B B (n+m))$ time using radix sort, with the first sorting-criterium being the length of strings (and the sorting being done decreasingly, from longest to shortest) and then the second criterium being their lexicographic value. Further, it is immediate that the solution to $\Problem{LRC-BR}$ is obtained by finding the first pair of consecutive strings $s_1$ and $s_2$ in the sorted list $S$, such that $s_1$ is a subsequence of one of the input words and $s_2$ of the other one and $s_1=s_2$. Hence $\Problem{LRC-BR}$ can be solved in $O(B 2^B (n + m))$. \qed
\end{proof}


